MCTensor: A High-Precision Deep Learning Library with Multi-Component Floating-Point

In this paper, we introduce MCTensor, a library based on PyTorch for providing general-purpose and high-precision arithmetic for DL training. MCTensor is used in the same way as PyTorch Tensor: we implement multiple basic, matrix-level computation operators and NN modules for MCTensor with identical PyTorch interface. Our algorithms achieve high precision computation and also benefits from heavily-optimized PyTorch floating-point arithmetic. We evaluate MCTensor arithmetic against PyTorch native arithmetic for a series of tasks, where models using MCTensor in float16 would match or outperform the PyTorch model with float32 or float64 precision.

==> algo/basic/GrowExpN.tex <==
\begin{algorithm}[H]
   \caption{\textbf{Grow-ExpN}}
   \label{alg:growexpn}
\begin{algorithmic}
\STATE {\bfseries Input:}  $nc$-MCTensor $x$, PyTorch Tensor $v$
   \STATE \textbf{initialize} $Q\leftarrow v$
   \FOR{$i=1$ to $nc$}
    \STATE $k\leftarrow nc+1-i$
    \STATE $(Q, h_k) \leftarrow \textbf{Two-Sum}(x_{k-1}, Q)$
   \ENDFOR
   \STATE $h  \leftarrow (Q,h_1,\cdots,h_{nc})$
   \STATE {\bfseries Return:} $\textbf{Simple-Renorm}(h, nc)$ 
\end{algorithmic}
\end{algorithm}

==> algo/basic/QTwoSum.tex <==
\begin{algorithm}[H]
   \caption{\textbf{Quick Two-Sum}}
   \label{alg:qtwosum}
   \begin{algorithmic}
      \STATE{\bfseries Input:} $p$-bit floats $a,b$, where $p \ge 3$
      \STATE $~~~~~~x\leftarrow\textbf{fl}(a+b)$
      \STATE $~~~~~~y\leftarrow\textbf{fl}(b-\textbf{fl}(s-a)$
      \STATE {\bfseries Return:} $(x,y)$
   \end{algorithmic}
\end{algorithm}

==> sections/2_Background.tex <==
\section{Related Work}
\wentao{1. high precision floats, what is bigfloat, usage of bigfloats and limitations. }

\TC{2. introduce mcf, some algorithms and guarantees proposed. requirements, orders decreasing, sum of multiple ordinary floats, advantages over bigfloat.
3.(double-double, quad-double)
existing work using mcf and how, quad-double, double-double library and other libraries, how many components, applications.}

\canal{4. applications that benefits from MCF, use MCF to achieve high precision training with low precision floats, hyperbolic space, the NaN problem, running with float64 to avoid nans, unbounded errors, why this is needed? }

% The followings are abstract from these papers.
% COPIED! Need to change 
% \cite{richard1997adaptive}
% The first is to offer fast software-level algorithms for exact addition and multiplication of arbitrary precision floating-point values. The second is to propose a technique for adaptive precision arithmetic that can often speed these algorithms when one wishes to perform multi-precision calculations that do not always require exact arithmetic, but must satisfy some error bound. The third is to use these techniques to develop implementations of several common geometric calculations whose required degree of accuracy depends on their inputs. These robust geometric predicates are adaptive; their running time depends on the degree of uncertainty of the result, and is usually small. These algorithms work on computers whose floating-point arithmetic uses radix two and exact rounding, including machines complying with the IEEE 754 standard. The inputs to the predicates may be arbitrary single or double precision floating-point numbers. C code is publicly available for the 2D and 3D orientation and incircle tests, and robust Delaunay triangulation using these tests. Timings of the implementations demonstrate their effectiveness.

% \cite{bailey2015high}
% Abstract: For many scientific calculations, particularly those involving empirical data, IEEE 32-bit floating-point arithmetic produces results of sufficient accuracy, while for other applications IEEE 64-bit floating-point is more appropriate. But for some very demanding applications, even higher levels of precision are often required. This article discusses the challenge of high-precision computation, in the context of mathematical physics, and highlights what facilities are required to support future computation, in light of emerging developments in computer architecture.


% \cite{fousse2007mpfr}
% This article presents a multiple-precision binary floating-point library, written in the ISO C language, and based on the GNU MP library. Its particularity is to extend to arbitrary-precision, ideas from the IEEE 754 standard, by providing correct rounding and exceptions. We demonstrate how these strong semantics are achieved---with no significant slowdown with respect to other arbitrary-precision tools---and discuss a few applications where such a library can be useful.


% %write-up [software implementations of high precision training]
High precision arithmetic were explored and implemented in many programming languages.  Bailey and Borwein \cite{bailey2015high} introduced the ongoing challenges for carrying the high precision computations, specifically in the area of mathematical physics.  Also, the software and hardware requirements for dealing with numerical difficulties were presented in light of emerging developments in computer architecture.  In this work\cite{fousse2007mpfr}, a multiple-precision binary floating-point library was presented.  The implementations were built on top of GNU MP library and the was programmed in ISO C language.    Through providing proper rounding and exceptions, the MPFR library can extend to arbitrary-precision from the IEEE 754 standard.  

% %what is MCF representation? Why we need them(high precision with limited precision)? Who(priest; Hida)?

A Multi-Component Floating Point Format is an unevaluated sum of multiple IEEE half/standard/double floating point numbers and can serve as a representation for higher precision floating point values.  Hida et al\cite{hida2001algorithms} showed that with a quadruple of double precision floating point values, precision of at least 212 bit of significand can be achieved.  In their work, there are also algorithms designed for carrying arithmetic operations (four basic operations and transcendental operations) in the Multi-Component format.  They also further demonstrated the extensive correctness of these algorithms.

% %QpyTorch, Revisiting BFloat16, low precision to achieve high precision training,
QPyTorch\cite{zhang2019qpytorch} is one example of utilizing low precision floating point values, for instance, Half Tensor(float16), for arithmetic simulation framework based on PyTorch. Specifically, QPyTorch was designed to investigate the area of low-precision training and to aid such study through simulation without hardware overhead.  Furthermore, to reduce the impact of simulator overhead, a fused-kernel approach was deployed and thus enabling study of large-scale problems with QPyTorch.  



%high precision learning on hyperbolic space


% \cite{zhang2019qpytorch}
% Low-precision training reduces computational cost and produces efficient models. Recent research in developing new low-precision training algorithms often relies on simulation to empirically evaluate the statistical effects of quantization while avoiding the substantial overhead of building specific hardware. To support this empirical research, we introduce QPyTorch, a low-precision arithmetic simulation framework. Built natively in PyTorch, QPyTorch provides a convenient interface that minimizes the efforts needed to reliably convert existing codes to study lowprecision training. QPyTorch is general, and supports a variety of combinations of precisions, number formats, and rounding options. Additionally, it leverages an efficient fused-kernel approach to reduce simulator overhead, which enables simulation of large-scale, realistic problems. QPyTorch is publicly available at
% COPIED
% \cite{cai2020zeroq}
% Quantization is a promising approach for reducing the inference time and memory footprint of neural networks. However, most existing quantization methods require access to the original training dataset for retraining during quantization. This is often not possible for applications with sensitive or proprietary data, e.g., due to privacy and security concerns. Existing zero-shot quantization methods use different heuristics to address this, but they result in poor performance, especially when quantizing to ultra-low precision. Here, we propose ZEROQ, a novel zero-shot quantization framework to address this. ZEROQ enables mixed-precision quantization without any access to the training or validation data. This is achieved by optimizing for a Distilled Dataset, which is engineered to match the statistics of batch normalization across different layers of the network. ZEROQ supports both uniform and mixed-precision quantization. For the latter, we introduce a novel Pareto frontier based method to automatically determine the mixed-precision bit setting for all layers, with no manual search involved. We extensively test our proposed method on a diverse set of models, including ResNet18/50/152, MobileNetV2, ShuffleNet, SqueezeNext, and InceptionV3 on ImageNet, as well as RetinaNet-ResNet50 on the Microsoft COCO dataset. In particular, we show that ZEROQ can achieve 1.71\% higher accuracy on MobileNetV2, as compared to the recently proposed DFQ [32] method. Importantly, ZEROQ has a very low computational overhead, and it can finish the entire quantization process in less than 30s (0.5\% of one epoch training time of ResNet50 on ImageNet). We have open-sourced the ZEROQ framework1.


% \cite{hida2007library}
% A double-double number is an unevaluated sum of two IEEE double precision numbers, capable of representing at least 106 bits of significand. Similarly, a quad-double number is an unevaluated sum of four IEEE double precision numbers, capable of representing at least 212 bits of significand. Algorithms for various arithmetic operations (including the four basic operations and various algebraic and transcendental operations) are presented. A C++ implementation of these algorithms is also described, along with its C and Fortran interfaces. Performance of the library is also discussed.

% \cite{bezanson2017julia}

% \cite{cuda}

% \cite{markidis2018nvidia}




% \cite{li2021unleashing}
% Li et al proposed QUANTENSOR to replace general-purpose tensor computations with low-precision quantized tensor computations on NVIDIA Tensor Cores, and they developed a residual-based precision refinement technique to control the quantization error. 
% Tensor-specialized hardware for supporting low precision arithmetic has become an inevitable trend due to
% the ever-increasing demand on computational capability and energy efficiency in intelligent applications. The main challenge faced when accelerating a tensor program on tensor-specialized hardware is how to achieve the best performance possible in reduced precision by fully utilizing its computational resources while keeping the precision loss in a controlled manner. In this paper, we address this challenge by proposing QUANTENSOR, a new approach for accelerating general-purpose tensor programs by replacing its tensor computations with low-precision quantized tensor computations on NVIDIA Tensor Cores. The key novelty is a new residual-based precision refinement technique for controlling the quantization errors, allowing tradeoffs between performance and precision to be made. Evaluation with GEMM, deep neural networks, and linear algebra applications shows that QUANTENSOR can achieve remarkable performance improvements while reducing the precision loss incurred significantly at acceptable overheads.


% \cite{sun2020ultra}
% In this paper, we propose a number of novel techniques and numerical representation formats that enable, for the very first time, the precision of training systems to be aggressively scaled from 8-bits to 4-bits. To enable this advance, we explore a novel adaptive Gradient Scaling technique (GradScale) that addresses the challenges of insufficient range and resolution in quantized gradients as well as explores the impact of quantization errors observed during model training. We theoretically analyze the role of bias in gradient quantization and propose solutions that mitigate the impact of this bias on model convergence. Finally, we examine our techniques on a spectrum of deep learning models in computer vision, speech and NLP. In combination with previously proposed solutions for 4-bit quantization of weight and activation tensors, 4-bit training shows non-significant loss in accuracy across application domains while enabling significant hardware acceleration (>7× over state of the art FP16 systems).

% hyperbolic space, embedding, the NaN problem

==> tables/MCBert.tex <==
    \begin{table*}[H]
     \centering
            \small\begin{tabular}{lcccr}
            \toprule
             Model & COLA & SST-B & MPRC & RTE \\
            \midrule
            \textbf{MCBert (nc=1)} & 0 & 0 & 0 & 0 \\
            \textbf{MCBert (nc=2)} & 0 & 0 & 0 & 0 \\
            \textbf{MCBert (nc=3)} & 0 & 0 & 0 & 0 \\
            \textbf{Bert (f16)} & 0 & 0 & 0 & 0 \\
            \textbf{Bert (f32)} & 0 & 0 & 0 & 0 \\
            \textbf{Bert (f64)} & 0 & 0 & 0 & 0 \\
        
            \bottomrule
            \end{tabular}
        \label{tab:mcbert}
    \end{table*}


==> tables/matrixOP.tex <==
\begin{table*}[htbp]
 \centering
    \caption{\centering  MCTensor Matrix Operators Running Time (mean $\pm$ sd) }
    \scalebox{0.8}{\small\begin{tabular}{lccccl} 
    \toprule
     Operators & Inputs sizes & FloatTensor & 1-MCTensor & 2-MCTensor & 3-MCTensor  \\
    \midrule
    \textbf{Dot-MCN} & $5000, 5000$ & $ 1.61\us\pm3.29\ns$ 
    & $ 442\us\pm5.61\us$
    & $ 656\us\pm1.16\us$
    & $ 858\us\pm12.2\us$\\                
\textbf{MV-MCN} & $(5000\times 500),500$    
& $ 157\us\pm4.32\us$
& $ 320\ms\pm5.78\ms$
& $ 460\ms\pm10.7\ms$
& $ 580\ms\pm12.1\ms$ \\
    \textbf{Matmul-MCN} & ( 500$\times$ 200), ( 200$\times$ 50)    
    & $ 97.3\us\pm1.1\us$
    & $ 495\ms\pm10.8\ms$
    & $ 735\ms\pm21.7\ms$
    & $ 934\ms\pm28\ms$ \\
    \bottomrule
    \end{tabular}}
    \label{tab:matrixop}
    \vspace{-1em}
\end{table*}


==> tables/mlpMNIST.tex <==
\begin{table}[ht]
 \centering
    \caption{\centering MCMLP Models on Reduced MNIST Dataset }
    \scalebox{0.85}{
        \small\begin{tabular}{lccr}
        \toprule
         Model & Training Loss & Testing accuracy   \\
        \midrule
        \textbf{MCMLP (f16 nc=1)} & _ \\
        \textbf{MCMLP (f16 nc=2)} & _ \\
        \textbf{MCMLP (f16 nc=3)} & _ \\
        \textbf{PyTorch MLP (f16)} & _ \\
        \textbf{PyTorch MLP (f32)} & _ \\
        \textbf{PyTorch MLP (f64)} & _ \\
    
        \bottomrule
        \end{tabular}
    }
    \label{tab:mlpMNIST}
\end{table}

